Efficient differentiable quadratic programming layers: an ADMM approach

Recent advances in neural-network architecture allow for seamless integration of convex optimization problems as differentiable layers in an end-to-end trainable neural network. Integrating medium and large scale quadratic programs into a deep neural network architecture, however, is challenging as solving quadratic programs exactly by interior-point methods has worst-case cubic complexity in the number of variables. In this paper, we present an alternative network layer architecture based on the alternating direction method of multipliers (ADMM) that is capable of scaling to problems with a moderately large number of variables. Backward differentiation is performed by implicit differentiation of the residual map of a modified fixed-point iteration. Simulated results demonstrate the computational advantage of the ADMM layer, which for medium scaled problems is approximately an order of magnitude faster than the OptNet quadratic programming layer. Furthermore, our novel backward-pass routine is efficient, from both a memory and computation standpoint, in comparison to the standard approach based on unrolled differentiation or implicit differentiation of the KKT optimality conditions. We conclude with examples from portfolio optimization in the integrated prediction and optimization paradigm.

==> sections/b_method/c_forward.tex <==
\section{Methodology} \label{sec:method}
\subsection{Mean-Variance Optimization}
We consider a universe of $d_z$ assets and denote the matrix of (excess) return observations as $\bY=[\by^{(1)},\by^{(2)},...,\by^{(m)} ] \in \mathbb{R}^{m\times d_z}$ with $m > d_z$. We define the portfolio $\bz \in \mathbb{R}^{d_z}$,  where the element, $\bz_i$, denotes the proportion of total capital invested in the $i^{\text{th}}$ asset. Therefore, for a particular return observation $\by^{(i)}$, the optimal portfolio weights, $\bz^*(\by^{(i)})$, is given by the solution to the following convex quadratic program:
\begin{equation}\label{eq:mvo_ineq}
\begin{split}
\minimize_z \quad &  -\bz^T \toi{ \by } + \frac{\delta}{2} \bz^T \toi{\bV} \bz \\
\text{subject to} \quad &   \bA \bz = \blb, \qquad \bG \bz \leq \bh\\
\end{split}
\end{equation}
where $\toi{ \bV }$ is a positive definite covariance matrix and $\delta \in \mathbb{R}_+$ is a risk-aversion parameter that controls the trade-off between minimizing variance and maximizing return.
%$\mathbb{F} = \{f \mid f(\bx,\btheta) = \btheta^T \bx\}$
In reality, we do not know the true value of $\toi{ \by }$ at decision time. We therefore estimate the values $\toi{ \by }$ through associated auxiliary variables $\toi {\bx } \in \mathbb{R}^{d_x}$. In this paper we consider regression based predictions models of the form:
$$\toi {\hat{\by} } =  \bbeta^T \toi {\bx} $$%f( \toi{ \bx },\bbeta)
where $\bbeta \in \mathbb{R}^{d_x \times d_y}$ is a matrix of regression coefficients. For simplicity, we consider a traditional parameter estimation process, and choose $\bbeta$ that minimizes the least-squares loss function $\ell(\by, \hat{\by}) = \lVert \by - \hat{\by} \rVert_2^2$.   Therefore, given training data set $\mathcal{D} = \{(  \toi{ \bx },  \toi{ \by } )\}_{i=1}^m$, we choose $\hat{\btheta}$ such that:
\begin{equation} \label{theta_hat}
\begin{split}
    \hat{\bbeta} & = \argmin_{  \bbeta }  \mathbb{E}_D[\ell (\bbeta^T \toi {\bx},  \toi{ \by } )],
\end{split}
\end{equation}
where $\mathbb{E}_\mathcal{D}$ denotes the expectation operator with respect to the training distribution $\mathcal{D}$.  The resulting least-squares estimators therefore given by:

\begin{equation} \label{eq:y_hat}
\begin{split}
\toi{\hat{  \by}} & =  \hat{\bbeta}^T  \toi{ \bx }\\
\toi{\hat{ \bV } } & = \hat{\bbeta}^T  \hat{\bW} \hat{\bbeta} + \hat{\bF},
\end{split}
\end{equation}
where $\hat{\bW }$  and  $\hat{\bF}$ denote the estimated covariance matrix of auxiliary variables and the diagonal matrix of residual variances, respectively. Note that in many applications, the eigenvalues of $\hat{\bF}$ are typically much smaller that that of $\hat{\bbeta}^T  \hat{\bW} \hat{\bbeta}$, and therefore the latter is a good low-rank approximation to the asset covariance matrix \citep{Goldfarb2003}. In practice, however, we note that the prediction model parameters, $\bbeta$, can easily be integrated and optimized by the stochastic optimization framework presented in Section \ref{sec:method_sof}.

Finally, under the regression estimation hypothesis, the mean-variance nominal objective (cost) function in Program $\eqref{eq:mvo_ineq}$  has the following form:
\begin{equation}\label{eq:mvo_cost_hat}
\begin{split}
c(\bz, \toi{\hat{\by}} )&  = -\bz^T \toi{ \hat{\by} } + \frac{\delta}{2} \bz^T \toi{\bV} \bz.
\end{split}
\end{equation}

\subsection{Motivation for Norm Penalty}
Augmenting Equation $\eqref{eq:mvo_cost_hat}$ with a norm penalty results in a standard PPQP, presented below:

\begin{equation}\label{eq:mvo_ineq_ppqp}
\begin{split}
\minimize_z \quad &  c_P(\bz, \toi{\hat{\by}},\btheta, \bgamma )\\
\text{subject to} \quad &   \bA \bz = \blb, \quad \bG \bz \leq \bh,
\end{split}
\end{equation}
where
\begin{equation}\label{eq:mvo_cost_hat}
\begin{split}
c_P(\bz, \toi{\hat{\by}},\btheta, \bgamma ) &  =-\bz^T \toi{ \hat{\by} } + \frac{\delta}{2} \bz^T \toi{\bV} \bz + P(\bz,\btheta,\bgamma).
\end{split}
\end{equation}
For simplicity, we have dropped the parameterization of all other objective and constraint variables. In the general case, however, these variables may also be parameterized and learnable and we provide such an example  in Section \ref{sec:results}.

Recall, $P(\bz,\btheta,\bgamma)$ is a convex combination of $L_1$ and $L_2$ norm penalties as defined in Equation $\eqref{eq:penalty}$. The choice of this specific norm penalty is deliberate and motivated by prior work that establishes the connection between norm penalized portfolio weights with covariance shrinkage and robust optimization.

\subsubsection{Covariance Shrinkage Estimator}
The linear covariance shrinkage estimator presented by \citet{Ledoit2003} is a convex combination of the sample covariance matrix, $\bV$ and a structured estimator $\bS$:
\begin{equation}\label{eq:shrink}
\hat{\bV} = (1 - \epsilon)\bV + \epsilon \bS = \bV + \epsilon (\bS - \bV),
\end{equation}
where $ 0 \leq \epsilon \leq 1$. From Equations $\eqref{eq:q_l2}$ and $\eqref{eq:q_approx}$, it is easy to see that our choice of norm penalty conforms to a linear  covariance shrinkage estimator. Specifically, for a particular choice of $\alpha$, $\bgamma_1$ and $\bgamma_2$, we have the following covariance shrinkage estimator:

\begin{equation}\label{eq:shrink_norm}
\hat{\bV} = \bV +  \alpha \bgamma_1 (\lVert \bE(\btheta)\bz^* \rVert_1 + \tau)^{-1} \bE(\btheta)^T \bE(\btheta) + (1 - \alpha) \bgamma_2 \bD(\btheta)^T\bD(\btheta),
\end{equation}
where $\bE(\btheta)^T \bE(\btheta) \succeq 0$ and $\bD(\btheta)^T\bD(\btheta) \succeq 0$ to ensure positive definiteness of $\hat{\bV}$.


\subsubsection{Robust Optimization}
Following \citet{Fabozzi2007}, we assume that the error in our estimate of expected returns is no larger than $\bgamma \geq 0$ and consider the following box uncertainty set:
\begin{equation}\label{eq:uncertainty_set_box}
\bU_{\by} = \{\by | \lVert \by_i - \bar{\by}_i \rVert_1 \leq \bgamma_i, i=1,...,d_y \}.
\end{equation}
The robust MVO counterpart is given as:
\begin{equation}\label{eq:mvo_ro}
\begin{split}
\minimize_z \quad &  \max_{\toi{ \by } \in \bU_{\by}}( -\bz^T \toi{ \by } ) + \frac{\delta}{2} \bz^T \toi{\bV} \bz \\
\text{subject to} \quad &   \bA \bz = \blb, \qquad \bG \bz \leq \bh\\
\end{split}
\end{equation}
%\quad & \bU_{\toi{\by}} = \{\toi{\by} | (\toi{\by} - \bar{\by})^T \bOmega^{-1} (\toi{\by} - \bar{\by}) \leq \kappa^2 \}
Under box uncertainty, Program $\eqref{eq:mvo_ro}$ simplifies to the following $L_1$-norm penalized quadratic program:
\begin{equation}\label{eq:mvo_ro_box}
\begin{split}
\minimize_z \quad &   -\bz^T \toi{ \by } + \bgamma^T \lvert \bz \rvert  +  \frac{\delta}{2} \bz^T \toi{\bV} \bz \\
\text{subject to} \quad &   \bA \bz = \blb, \qquad \bG \bz \leq \bh
\end{split}
\end{equation}
It is then easy to verify that Program $\eqref{eq:mvo_ro_box}$ is an $L_1$-norm PPQP with sparsifying matrix ${\bE(\btheta) = \diag(\bgamma) }$.


Alternatively, following \citet{Ceria2006} we now consider the ellipsoidal uncertainty set on the vector of expected returns:
\begin{equation}\label{eq:uncertainty_set}
\bU_{\by} = \{\by | (\by - \bar{\by})^T \bOmega^{-1} (\by - \bar{\by}) \leq \kappa^2 \},
\end{equation}
where $\bOmega$ is a symmetric positive-definite uncertainty matrix and $\kappa^2$ defines the level of uncertainty. %Following \citet{Yin2019}, the robust MVO counterpart to Program $\eqref{eq:mvo_ineq}$ is given as:

%\begin{equation}\label{eq:mvo_ro}
%\begin{split}
%\minimize_z \quad &  \max_{\toi{ \by } \in \bU_{\by}}( -\bz^T \toi{ \by } ) + \frac{\delta}{2} \bz^T \toi{\bV} \bz \\
%\text{subject to} \quad &   \bA \bz = \blb, \qquad \bG \bz \leq \bh\\
%\quad & \bU_{\toi{\by}} = \{\toi{\by} | (\toi{\by} - \bar{\by})^T \bOmega^{-1} (\toi{\by} - \bar{\by}) \leq \kappa^2 \}
%\end{split}
%\end{equation}
Under ellipsoidal uncertainty, Program $\eqref{eq:mvo_ro}$ simplifies to the following constrained second-order cone program:
\begin{equation}\label{eq:mvo_ro_simp}
\begin{split}
\minimize_z \quad &   -\bz^T \toi{ \by } + \frac{\delta}{2} \bz^T \toi{\bV} \bz \\
\text{subject to} \quad &   \bA \bz = \blb, \qquad \bG \bz \leq \bh\\
\quad & \lVert \bOmega^{\frac{1}{2} } \bz \rVert_2  \leq \kappa
\end{split}
\end{equation}
Relaxing the second-order cone constraint and following the results presented in \citet{Zhu2009}, it follows that there exits a $\bgamma_2 \geq 0$ such that the following Program is equivalent to Program $\eqref{eq:mvo_ro_simp}$:
\begin{equation}\label{eq:mvo_ro_simp_relax}
\begin{split}
\minimize_z \quad &   -\bz^T \toi{ \by } + \frac{\delta}{2} \bz^T \toi{\bV} \bz + \bgamma_2 \lVert \bOmega^{\frac{1}{2} } \bz \rVert_2^2 \\
\text{subject to} \quad &   \bA \bz = \blb, \qquad \bG \bz \leq \bh.
\end{split}
\end{equation}
It is easy to see that Program $\eqref{eq:mvo_ro_simp_relax}$ is an $L_2$ norm PPQP with uncertainty structure $\bD(\btheta) = \bOmega^{\frac{1}{2}}$.


\subsubsection{Regularized Least-Squares}
We re-cast the mean-variance Program $\eqref{eq:mvo_ineq}$ as a constrained ordinary least-squares problem under the sample moment estimation hypothesis:
\begin{equation}\label{eq:mvo_ols}
\begin{split}
\minimize_z \quad & \frac{1}{2m}\lVert \bz^T(\bY - \bar{\bY})  - \bone_{m}  \rVert_2^2 \\
\text{subject to} \quad &   \bA \bz = \blb, \qquad \bG \bz \leq \bh\\
\end{split}
\end{equation}
where $\bar{\bY}$ denotes the sample mean of asset returns and $\bone_{m} \in \mathbb{R}^{m}$ is a vector of ones.
If we augment Program $\eqref{eq:mvo_ols}$ with the elastic net penalty:
\begin{equation}\label{eq:penalty_simp}
\begin{split}
P_{EN}(\bz,\bgamma) = \alpha \bgamma_1 \lVert \bz \rVert_1 + (1 - \alpha) \frac{\bgamma_2}{2} \lVert \bz \rVert_2^2
\end{split}
\end{equation}
then Program $\eqref{eq:mvo_ols}$ is a constrained regularized ordinary least-squares problem with regression coefficients $\bz$. When $\alpha = 0$ then Program $\eqref{eq:mvo_ols}$ conforms to a constrained ridge regression for regularization of multiple regression problems that are ill-posed or suffer from issues of multi-collinearity \cite{Tikhonov1963}. MVO portfolio are also susceptible to these forms of model misspecification effects, such as when the asset universe under consideration is large or contains securities with structurally similar underlying economic drivers. For these reasons, we posit that MVO would benefit from some form of ridge regression regularization.
% In many situations in portfolio management,
% particularly when the asset universe under consideration is large and contains many
%may also suffer from  are equally as vulnerable to In MVO portfolioSuch issues are common to portfolio optmization, assets

Similarly, when $\alpha = 1$ then Program $\eqref{eq:mvo_ols}$ conforms to the well-known constrained lasso regression, commonly used for best-subset feature selection and for targeting sparse solutions to multiple regression problems \citep{Tibshirani1996}. In many regression situations, particularly in low signal-to-noise ratio regimes, a parsimonious solution is often preferred for mitigating model overfit\citep{Hastie2017}. It is often the case that MVO portfolios are constructed with prediction models that have very low signal-to-noise ratios. It follows, therefore, that MVO would also benefit from a lasso-styled regularization by removing these low signal-to-noise ratio assets from the portfolio - thus providing a more parsimonious portfolio construction process.% that provide insufficiently strong predictability.% have sufficiently low, It follows therefore that MVO would also benefit from lasso regularization; in particular by reSimilarly Again such problems are frequently encounter removes assets for which our prediction model is poor predictor

%in many regression situations with low signal-to-noise ratios for In many regression situations, sparse solution is generally preferred since you can explain your model in terms of just a few variables. parsimonous, avoids overfit, removes redundant or non-explanatory features.

%Show MVO is a ols problem.
%As lasso equivalent.

%A sparse solution is generally preferred since you can explain your model in terms of just a few variables. parsimonous, avoids overfit, removes redundant or non-explanatory features.
%removes assets for which our prediction model is poor


==> sections/b_method/d_backward.tex <==
\subsection{Stochastic Optimization Framework}\label{sec:method_sof}
As stated in Section \ref{sec:intro}, the norm penalty parameters $\btheta$ and $\bgamma$ are typically selected by heuristic cross-validation or resampling methods. Here, we follow the work of \citet{Butler2021IPOb,Butler2020IPO} and present a stochastic optimization framework for optimizing norm penalty parameters in the context of the final decision-based optimization, its inputs and constraints.

Specifically, we are interested in optimizing $\btheta$ and $\bgamma$ in the context of the norm penalized mean-variance cost, $c_P$, and its constraints, $\mathbb{Z} = \{ \bz \in \mathbb{R}^{d_z} | \bA \bz = \blb, \bG \bz \leq \bh \}$, in order to minimize the average realized nominal cost of the policy $ \bz^*( \toi{\hat{\by}},  \btheta, \bgamma)$ induced by this parameterization. For a fixed instantiation  $( \toi{\hat{\by}}, \btheta, \bgamma)$, we solve Program $\eqref{eq:mvo_ineq_ppqp}$ in order to determine the optimal portfolio weights:
\begin{equation} \label{eq:z_star}
\begin{split}
  \bz^*(\toi{\hat{\by}}, \btheta, \bgamma) &  = \argmin_{ \bz \in \mathbb{Z}}  c_P( \bz,  \toi{\hat{\by}},\btheta, \bgamma ).
 \end{split}
\end{equation}
Our objective is to therefore choose $\btheta$ and $\bgamma$ in order to minimize the average realized nominal cost, $c$, induced by the decision policy $\bz^*(\toi{\hat{\by}}, \btheta, \bgamma)$. The resulting problem can be posed as a stochastic optimization problem, presented in program $\eqref{eq:stoch_program}$.
\begin{equation} \label{eq:stoch_program}
\begin{split}
\minimize_{ \btheta, \bgamma }  & \quad  \mathbb{E}_\mathcal{D}[ c( \bz^*(  \hat{\by}, \btheta, \bgamma), \by) ] \\
\text{subject to } & \quad    \bz^*(\hat{\by}, \btheta, \bgamma)  = \argmin_{ \bz \in \mathbb{Z}}  c_P( \bz,  \hat{\by},\btheta, \bgamma )\\
& \quad \bgamma \geq 0.
\end{split}
\end{equation}
In practice, we are typically presented with discrete observations $ \mathcal{D} = \{( \bx^{(i)}, \by^{(i)})\}_{i=1}^m$ and therefore we can approximate the expectation by its sample average approximation \citep{Shapiro2009}. The full discrete stochastic optimization program is presented in program $\eqref{eq:stoch_discrete}$:
\begin{equation} \label{eq:stoch_discrete}
\begin{split}
\minimize_{ \btheta, \bgamma } \quad & \frac{1}{m} \sum_{i=1}^m c(\bz^*(  \toi{\hat{\by}}, \btheta, \bgamma), \by^{(i)})  \\
\text{subject to } & \quad   \bz^*(\toi{\hat{\by}}, \btheta, \bgamma)  = \argmin_{\bz \in \mathbb{Z}}  c_P( \bz,  \toi{\hat{\by}},\btheta, \bgamma ) \quad \forall i \in 1,...,m\\
& \quad \bgamma \geq 0.
\end{split}
\end{equation}

Observe that the stochastic optimization framework  results in a complicated dependency of the parameters, $\btheta$ and $\bgamma$, on the optimized values, $\bz^*(\hat{\by}, \btheta, \bgamma)$, connected through the $\argmin$ function. Fortunately, the implicit differentiation techniques, described in detail in Section \ref{sec:background}, provide an efficient routine for computing the gradient of the nominal cost with respect to all relevant problem variables. We propose optimizing the penalty parameters by first-order gradient descent in an end-to-end differentiable neural network, depicted in Figure \ref{fig:network}. Note that the prediction model parameters, $\bbeta$, can also be readily optimized by the stochastic optimization framework; resulting in a fully integrated predict and optimize framework (IPO).  For more detail we refer the reader to \citet{Butler2021IPOb, Butler2020IPO}.% The resulting stochastic optimaization work-flow is depicted in Figure \ref{fig:network}.

\begin{figure}[H]
\centering
\begin{tikzpicture}[
    node distance = 5mm and 7mm,
      start chain = going right,
  alg/.style = {draw, align=center, font=\linespread{0.8}\selectfont, minimum width={width("Backward Pass Algo:")+12pt}}
                    ]
\begin{scope}[every node/.append style={on chain, join=by -Stealth}]
%\node (n0) [alg] { Forward:   };
\node (n1) [alg] {$ \phantom{f} $ \\ $\quad \bx^{(i)} \quad $ \\ $ $};
\node (n2) [alg]  {$\hat{\by}^{(i)} = \bbeta^T \bx^{(i)}$ \\ $ $ \\ $\bD( \btheta ),\bE( \btheta ), \bgamma$  };
\node (n3) [alg]  {$ \phantom{f} $ \\ $\min_{\bz} c_P( \bz,  \toi{\hat{\by}}, \btheta, \bgamma )$ \\ $ $};
\node (n4) [alg] {$ \phantom{f} $ \\ $c(\bz^*, \by^{(i)})$ \\ $ $ };
\end{scope}

\node[above=of n1]  {\underline{Input layer}};
\node[above=of n2]  {\underline{Predictive layer}};
\node[above=of n3]  {\underline{QP layer}};
\node[above=of n4]  {\underline{Loss Function}};
\end{tikzpicture}

\begin{tikzpicture}[
    node distance = 5mm and 7mm,
      start chain = going left,
  alg/.style = {draw, align=center, font=\linespread{0.8}\selectfont, minimum width={width("Backward Pass Algo:")+12pt} }
                    ]
\begin{scope}[every node/.append style={on chain, join=by -Stealth}]
\node (n4) [alg] {$ \phantom{f} $ \\ $\partial c / \partial \bz^*$ \\ $ $   };
\node (n3) [alg]  {$\partial \bz^* / \partial \hat{\by}, \partial \bz^* / \partial \bgamma  $ \\ $\partial \bz^* / \partial \bD( \btheta ) $ \\ $\partial \bz^* / \partial \bD( \btheta )$};
\node (n2) [alg]  {$ \partial \hat{\by}/ \partial \bbeta$ \\$\partial \bD( \btheta ) / \partial \btheta $\\ $\partial \bE( \btheta ) / \partial \btheta $};
\node (n1) [alg] {$\bbeta \leftarrow \bbeta - \bm g_\beta$ \\$\btheta \leftarrow \btheta - \bm g_\theta   $\\$\bgamma \leftarrow \bgamma - \bm g_\gamma   $};
%\node (n0) [alg] {Backward:};

\end{scope}

\end{tikzpicture}
\caption{Stochastic optimization framework represented as an end-to-end neural-network with predictive model layer, differentiable quadratic programming layer and realized nominal cost loss function. }
\label{fig:network}
\end{figure}
Lastly, we choose to search for locally optimal solutions by stochastic gradient descent (SGD). The descent direction, $\bm g_\theta$, at each iteration approximates the gradient of the nominal cost with respect to $\btheta$ and is given by :
$$
\bm g_\theta = \sum_{i\in B}\Big( \frac{\partial c   }{\partial \btheta} \Big)_{\mid (\bz^*(\toi{\hat{\by}}),\toi{\by} )}
$$
where in standard stochastic gradient descent, $B$ represents a randomly drawn sample batch.


%
% In the forward pass, the input layer takes the auxiliary variables $\bx^{(i)}$ and passes them to a simple linear layer to produce the estimates, $\hat{\by}^{(i)}$. The linear layer is either single connected, in the univariate case, or fully-connected, in the multivariate case. The predictions are then passed to a differentiable quadratic programming layer which, for a given input $\hat{\by}^{(i)}$, solves the nominal program and returns the optimal portfolio weights $\bz^*(\bx^{(i)},\btheta).$ At this point, we cache the factorized left-hand side matrix at the optimal solution, which will be invoked during backpropagation. Finally, the quality of the portfolio weights are evaluated by the cost function, $c(\bz^*(\bx, \btheta), \by^{(i)})$ in the context of the realized (true)  $\by^{(i)}.$
%
% The backpropagation algorithm computes the partial derivatives in the regular fashion in order to generate the gradient of the realized cost with respect to the regression coefficients. In the case of the QP layer, we are given as input the derivative of the realized cost with respect to the optimal weights: $\frac{\partial c}{\partial \bz^*}$. Following \citet{Amos2017}, we apply the implicit function theorem and compute $\frac{\partial c}{\partial \by}$ by multiplying the backward pass vector by the inverse of the transposed left-hand-side matrix, as shown in equation $\eqref{eq:diff_sol}$. Recall, we have cached the factorized left-side matrix and thus the gradient $\frac{\partial c}{\partial \by}$ is effectively provided at no additional computation cost.
%
%
%
%
%







